Domain Adaptation for Camera-Specific Image Characteristics using Shallow Discriminators

Each image acquisition setup leads to its own camera-specific image characteristics degrading the image quality. In learning-based perception algorithms, characteristics occurring during the application phase, but absent in the training data, lead to a domain gap impeding the performance. Previously, pixel-level domain adaptation through unpaired learning of the pristine-to-distorted mapping function has been proposed. In this work, we propose shallow discriminator architectures to address limitations of these approaches. We show that a smaller receptive field size improves learning of unknown image distortions by more accurately reproducing local distortion characteristics at a low network complexity. In a domain adaptation setup for instance segmentation, we achieve mean average precision increases over previous methods of up to 0.15 for individual distortions and up to 0.16 for camera-specific image characteristics in a simplified camera model. In terms of number of parameters, our approach matches the complexity of one state of the art method while reducing complexity by a factor of 20 compared to another, demonstrating superior efficiency without compromising performance.

==> images/ablation_simple_cam_ap_group.tex <==
\nextgroupplot[
legend style={
	at={(1.1,+0.5)},
	anchor=west,
	align=left,
	fill=none,
	legend columns=4,
	transpose legend,
},
xlabel={Model},
xmin=2,
xmax=7,
xtick={7,6,5,4,3,2},
xticklabels={A, B, C, D, E, F}, % inserted labels for idxs column xtick={7,6,5,4,3,2}
x dir=reverse,	
]
\newcommand{\degrad}{simple_cam_jpeg}
\newcommand{\testqpstr}{idx}
\addplot[semithick, dashed, col1]table{%
	0 0.3458739657843787
	100 0.3458739657843787
};
\addlegendentry{\textbf{Undistorted}}
\addplot[semithick, col1, mark=square*, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_none-baseline_testDistorted_ap.csv};
\addlegendentry{\textbf{Baseline}};
\addplot[semithick, col2, mark=*, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_none-oracle_testDistorted_ap.csv};
\addlegendentry{\textbf{Oracle}};
\addplot[semithick, col3, mark=asterisk, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_icip22_testDistorted_ap.csv};
\addlegendentry{\textbf{\discrThreeLay{}~\cite{Gruber2022}}};
\addplot[semithick, col6, mark=asterisk, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_arruda22_testDistorted_ap.csv};
\addlegendentry{\textbf{\arruda{}~\cite{Arruda2022}}};
% Ablation
\addplot[semithick, col7, mark=diamond, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_cut_netD-n_layers-3_L_nce-1_testDistorted_ap.csv};
\addlegendentry{\textbf{BD-A}};
\addplot[semithick, col8, mark=diamond, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_cut_netD-n_layers-2_L_nce-1_testDistorted_ap.csv};
\addlegendentry{\textbf{SD-A}};
\addplot[semithick, col9, mark=diamond, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_cut_netD-n_layers-1_L_nce-1_testDistorted_ap.csv};
\addlegendentry{\textbf{ESD-A}};

==> images/ap_group_template.tex <==
% Undistorted
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendimage{empty legend}
	\addlegendentry{Train: No distortion\\Test: No distortion}
}{}
\addplot[semithick, dashed, col1]table{%
	0 0.3458739657843787
	100 0.3458739657843787
};
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendentry{\textbf{Undistorted}}
	\addlegendimage{empty legend}
	\addlegendentry{}
}{}
%
% Baseline
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendimage{empty legend}
	\addlegendentry{Train: No distortion\\Test: Unknown distortion}
}{}
\addplot[semithick, col1, mark=square*, mark size=1, mark options={solid}]table[x=test_qp, y=ap, col sep=comma]{csvs/\degrad_none-baseline_testDistorted_ap.csv};
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendentry{\textbf{Baseline}};
	\addlegendimage{empty legend}
	\addlegendentry{}
}{}
%
% Oracle
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendimage{empty legend}
	\addlegendentry{Train: Unknown distortion\\Test: Unknown distortion}
}{}
\addplot[semithick, col2, mark=*, mark size=1, mark options={solid}]table[x=test_qp, y=ap, col sep=comma]{csvs/\degrad_none-oracle_testDistorted_ap.csv};
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendentry{\textbf{Oracle}};
	\addlegendimage{empty legend}
	\addlegendentry{}
}{}
% ICIP22
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendimage{empty legend}
	\addlegendentry{Train: Emulated distortion\\Test: Unknown distortion}
}{}
\addplot[semithick, col3, mark=asterisk, mark size=1, mark options={solid}]table[x=test_qp, y=ap, col sep=comma]{csvs/\degrad_icip22_testDistorted_ap.csv};
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendentry{\textbf{\discrThreeLay{}~\cite{Gruber2022}}};
}{}
%
% Arruda22
\addplot[semithick, col6, mark=asterisk, mark size=1, mark options={solid}]table[x=test_qp, y=ap, col sep=comma]{csvs/\degrad_arruda22_testDistorted_ap.csv};
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendentry{\textbf{\arruda{}~\cite{Arruda2022}}};
}{}
\addplot[semithick, col4, mark=x, mark size=1, mark options={solid}]table[x=test_qp, y=ap, col sep=comma]{csvs/\degrad_netD-n_layers-2_id-0-5_testDistorted_ap.csv};
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendentry{\textbf{\hspace*{0.19em}\discrTwoLay{} (ours)}}
}{}
\addplot[semithick, col5, mark=+, mark size=1, mark options={solid}]table[x=test_qp, y=ap, col sep=comma]{csvs/\degrad_netD-n_layers-1_id-0-5_testDistorted_ap.csv};
\ifthenelse{\equal{\degrad}{j2k}}{
	\addlegendentry{\textbf{\hspace*{0.19em}\discrOneLay{} (ours)}}
}{}
%

==> images/blur_gauss_ap_group.tex <==
\nextgroupplot[
xlabel={\blurQP},
xmin=1,
xmax=7,
xtick={1,3,5,7},
xticklabels={$1$,$3$,$5$,$7$},
title={Blur},
]
\newcommand{\degrad}{blur_gauss}
%
\input{images/ap_group_template.tex}

==> images/heif_ap_group.tex <==
\nextgroupplot[
xlabel={\heifQP},
xmin=27,
xmax=47,
xtick={27,32,...,47},
title={HEIF},
]
\newcommand{\degrad}{heif}
%
\input{images/ap_group_template.tex}

==> images/j2k_ap_group.tex <==
\nextgroupplot[
legend style={
	at={(1.3,-0.55)},
	anchor=west,
	align=left,
	fill=none,
},
xlabel={\jkQP{} in \si{\decibel}},
x dir=reverse,
xmin=30,
xmax=38,
xtick={38,36,...,30},
xticklabels={$38$,$36$,$34$,$32$,$30$},
title={JPEG2000},
]
%%
\newcommand{\degrad}{j2k}
%
\input{images/ap_group_template.tex}

==> images/jpeg_ap_group.tex <==
\nextgroupplot[
xlabel={\jpegQP},
x dir=reverse,
xmin=14,
xmax=42,
xtick={14,18,26,34, 42},
title={JPEG},
]
\newcommand{\degrad}{jpeg}
%
\input{images/ap_group_template.tex}

==> images/noise_gauss_ap_group.tex <==
\nextgroupplot[
xlabel={\noiseQP{}},
xmin=5,
xmax=50,
xtick={5,10,20,30,50},
xticklabels={$5$,$10$,$20$,$30$, $50$},
title={\ac{AWGN}},
]
\newcommand{\degrad}{noise_gauss}
%
\input{images/ap_group_template.tex}

==> images/simple_cam_ap_group.tex <==
\nextgroupplot[
xlabel={Model},
xmin=2,
xmax=7,
xtick={7,6,5,4,3,2},
xticklabels={A, B, C, D, E, F}, % inserted labels for idxs column xtick={7,6,5,4,3,2}
x dir=reverse,	
title={Simplified Camera},
]
\newcommand{\degrad}{simple_cam_jpeg}
\newcommand{\testqpstr}{idx}
%
% Undistorted
\addplot[semithick, dashed, col1]table{%
	0 0.3458739657843787
	100 0.3458739657843787
};
%
% Baseline
\addplot[semithick, col1, mark=square*, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_none-baseline_testDistorted_ap.csv};
%
% Oracle
\addplot[semithick, col2, mark=*, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_none-oracle_testDistorted_ap.csv};
%
% ICIP22
\addplot[semithick, col3, mark=asterisk, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_icip22_testDistorted_ap.csv};
% Arruda22
\addplot[semithick, col6, mark=asterisk, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_arruda22_testDistorted_ap.csv};
%
% New plots
\addplot[semithick, col4, mark=x, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_netD-n_layers-2_id-0-5_testDistorted_ap.csv};
\addplot[semithick, col5, mark=+, mark size=1, mark options={solid}]table[x=\testqpstr, y=ap, col sep=comma]{csvs/\degrad_netD-n_layers-1_id-0-5_testDistorted_ap.csv};
%

==> images/visuals_template_simple_cam_transposed.tex <==
%simple_cam_jpeg
\newcommand{\degrad}{simple_cam_jpeg}
\newcommand{\modelgroup}{00_true_dist}
%		
\newcommand{\qp}{1}
\node (imA-row1) at (0,0) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
\renewcommand{\qp}{9}
\node[align=center, right=-.18cm of imA-row1.east] (imC-row1) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
\renewcommand{\qp}{3}
\node[align=center, right=-.18cm of imC-row1.east] (imF-row1) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
%
\renewcommand{\modelgroup}{icip22}
%		
\renewcommand{\qp}{1}
\node[align=center, below=-.18cm of imA-row1.south] (imA-row2) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
\renewcommand{\qp}{9}
\node[align=center, right=-.18cm of imA-row2.east] (imC-row2) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
\renewcommand{\qp}{3}
\node[align=center, right=-.18cm of imC-row2.east] (imF-row2) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
%
\renewcommand{\modelgroup}{arruda22}
%		
\renewcommand{\qp}{1}
\node[align=center, below=-.18cm of imA-row2.south] (imA-row3) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
\renewcommand{\qp}{9}
\node[align=center, right=-.18cm of imA-row3.east] (imC-row3) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
\renewcommand{\qp}{3}
\node[align=center, right=-.18cm of imC-row3.east] (imF-row3) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
% 
\renewcommand{\modelgroup}{netD-n_layers-2_id-0-5}
%		
\renewcommand{\qp}{1}
\node[align=center, below=-.18cm of imA-row3.south] (imA-row4) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
\renewcommand{\qp}{9}
\node[align=center, right=-.18cm of imA-row4.east] (imC-row4) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
\renewcommand{\qp}{3}
\node[align=center, right=-.18cm of imC-row4.east] (imF-row4) {\includegraphics[trim=0 55 0 20,clip,width=\mywidth]{\impath{\degrad}{\qp}{\imname}{\cropnum}{\modelgroup}}};
%						
%%% add caption node
\node [font=\myfontsize, align=center, below=-.1cm of imA-row4.south] (imAcap)  {Model A};
\node [font=\myfontsize, align=center, below=-.1cm of imC-row4.south] (imCcap)  {Model C};
\node [font=\myfontsize, align=center, below=-.1cm of imF-row4.south] (imEcap)  {Model F};
%%
%% add caption node
\node [font=\myfontsize, align=center, left=0cm of imA-row1.west] (imArow) {True};
\node [font=\myfontsize, align=center, left=0cm of imA-row2.west] (imBrow) {\discrThreeLay{}~\cite{Gruber2022}};
\node [font=\myfontsize, align=center, left=0cm of imA-row3.west] (imCrow) {\arruda{}~\cite{Arruda2022}};
\node [font=\myfontsize, align=center, left=0cm of imA-row4.west] (imDrow) {\discrTwoLay{} (ours)};
